CSI: Contrastive Data Stratification for Interaction Prediction and its Application to Compound-Protein Interaction Prediction

Accurately predicting the likelihood of interaction between two objects (compound-protein sequence, user-item, author-paper, etc.) is a fundamental problem in Computer Science. Current deep-learning models rely on learning accurate representations of the interacting objects. Importantly, relationships between the interacting objects, or features of the interaction, offer an opportunity to partition the data to create multi-views of the interacting objects. The resulting congruent and non-congruent views can then be exploited via contrastive learning techniques to learn enhanced representations of the objects.

==> not_used.tex <==
Intro:

%Predicting the interaction between two sets of entities, modeled as the relationship between these entities, is a fundamental problem in Computer Science. An interaction could be a label-image pair, or a viewer-movie pair, or an author-paper pair, or a compound-protein pair. There are several methods to predict such relationships, but interaction prediction is the basic problem that needs to be solved in all these methods.

%Interpreting interactions as edges in a graph enables the interaction prediction problem to be modeled as a link prediction problem in social networks \citep{DAUD2020102716}. Annotation of text on images has also been modeled as an interaction prediction problem \citep{adnan2021automatic} by modeling the interaction as the text that goes with the given image. Recommender systems between users/entities and items to be recommended such as papers \citep{beel2016paper} and movies \citep{walek2020hybrid} can also be modeled as interaction prediction problems. A recommender system essentially makes recommendations by predicting the most likely pair that satisfies the relationship (interaction) given prior knowledge about known interactions. In this paper, we propose a general method to stratify data and predict interactions. To demonstrate our method, we will focus on the problem of compound-protein interaction prediction, where interactions are defined as the binding between a compound-protein pair.

%Predicting compound-protein interactions is an important pre-requisite for discovering drug targets, understanding human microbiome co-metabolism, understanding diseases like cancer and many other biological applications. Despite numerous advances in high-throughput screening, experimental methods for drug discovery still remain very expensive \citep{sinha2018drug},  necessitating the application of computational methods to predict compound-protein and molecule-enzyme interactions. The most common methods applied to this problem these days are end-to-end Deep Learning methods. In these methods, the molecule and the protein sequence are both converted into embeddings using a variety of techniques. Embeddings are real-valued vectors of a specific dimension representing the input. These embeddings are learnable and during training learn specific features of the input. The molecule embeddings can be generated using molecular fingerprints \citep{feng2018padme, lin2020deepgs, lee2019deepconv}. Another common method is to generate the molecule embeddings using Graph Neural Networks \citep{tsubaki2019compound, nguyen2021graphdta, ozturk2019widedta}. Similarly, protein embeddings can be created using fingerprints \citep{feng2018padme}. Deep learning models like CNN \citep{ozturk2018deepdta, lee2019deepconv}, and even transformers \citep{min2021pre, huang2021moltrans} have also been used to generate embeddings for proteins. The goal of all these models is to generate high quality embeddings for the molecules and the proteins to improve the downstream task of interaction prediction. Prior to deep learning methods, earlier methods that have been applied to this problem have been 3d docking simulations using physics based models for determining the binding modes \citep{decherchi2020thermodynamics}. Similarity based methods involve forming similarity based bipartite graphs to allow prediction of unknown interactions \citep{perlman2011combining, shi2015predicting} modeled as edges in the graph. Network based methods have applied similarity techniques across an entire network \citep{bagherian2021machine, thafar2020dtigems+, zeng2020network, luo2017network}. Recommender system  solutions map the interactions onto a sparse interaction matrix and apply matrix factorization as well as collaborative filtering methods \citep{bagherian2021machine, li2022boost, zhang2020graph, chen2021neural} to fill the interaction matrix for unknown interactions. However, traditional recommender systems suffer from the cold start problem \citep{wei2017collaborative} because of their inability to handle objects unseen during training. Hence interaction prediction using deep learning methods offer better alternatives because of their ability to handle unseen data.

%Deep-learning methods to predict interaction  broadly perform two main tasks: representation learning to learn representations of compounds and proteins, and using these learned representations for interaction prediction. The seminal paper \citep{bengio2013representation} articulates very well the challenges of representation learning - lack of availability of a smooth prior, shared features across tasks, input factor dependencies etc. These challenges can be further exacerbated by an end to end learning approach where the representation and the downstream task are learnt at the same time. Various model architectures like GAN, Encoder-Decoder, Autoencoders etc have been proposed for representation learning \citep{guo2019deep} which focus on learning both uni-modal as well as multi-modal representations in a joint latent space if required by the downstream task. For interaction prediction problem, where the data is inherently bifurcated by whether an interaction exists or not, contrastive learning lends itself very well as a viable option for representation learning \citep{le2020contrastive}. In fact since contrastive learning looks at interacting and non-interacting data simultaneously, a contrastive learning model trains a discriminative model based on the notion of mutual information inherent in the data. As such contrastive learning is a self-learning approach.

%To apply a method like Contrastive Multiview Coding (CMC) \citep{tian2020contrastive} to interaction data, we need to first create congruent (i.e. views of data sharing some common information) and non-congruent views of the data. Interaction data usually has many-to-many relationships among data objects. These many-to-many relationships allow for the interaction data to be stratified into congruent views for each object - the object itself is one view and all other objects related to it are another view. For some interaction networks, auxiliary data may also be available that allows other alternative ways to stratify the data. A common example of an interaction network is a viewer-movie network. Each viewer could be associated with multiple movies, and vice versa, allowing for views to be created for each viewer or for each movie. Additionally, auxiliary data like theater, location, year etc might be available for a viewer-movie network which can also be used as stratification keys for the data. 

%The key contribution of this paper is a method called \textbf{C}ontrastive Data \textbf{S}tratification for \textbf{I}nteraction Prediction - CSI - that can be used to stratify any interaction data hence making our method quite generalizable. Our method involves creating \textit{congruent} views of the data - containing all the data elements that share some mutual information - e.g. all proteins interacting with a given compound, or all compounds interacting with a given protein. In the first case, the original compound becomes one view of the data, and all proteins interacting with the compound become a different view of the data. The converse holds true for the second case. All views of the same datum created in this manner are \textit{congruent} views, and by implication, the views of any two different datum are \textit{non-congruent} with each other. 
%Once the data has been stratified into congruent and non-congruent views, we use a model based on Contrastive Multiview Coding (CMC) to utilize the stratified data in the representation learning task and learn better embeddings relevant for interaction prediction. The fundamental goal of CMC is to \textit{maximize} the \textit{mutual information} present in \textit{different congruent views} of the \textit{same data}. The mutual information existing in different views of the same data represents features of the data that are important for the downstream task. Hence maximizing the mutual information would create embeddings of the data that are rich in features suitable for the downstream task of interaction prediction. In CMC, the mutual information maximization is done by choosing a loss function such that the embeddings of congruent views of the \textit{same} data are pushed closer to each other in the embedding space, and are pushed away from embeddings of non-congruent views as shown in Figure \ref{fig:contrast}. Once representations have been learnt using CMC, these are used in the interaction prediction task for learning the final predictor. We also show how auxiliary information, if available,  can be used as a stratification key for the data. 


%The current methods for compound-protein interaction prediction have been generally applied to two widely accepted datasets KIBA \citep{tang2014making} and DAVIS \citep{davis2011comprehensive}. These datasets are small, and do not represent enzymatic reactions or drug-target interactions well. Molecule-protein datasets generally come in two flavors - interaction datasets which only document the known interactions between compounds and proteins, and reaction datasets which document complete reactions from substrates to products, catalyzed by enzymes. To demonstrate the generalizability of our method, we use both enzymatic and non-enzymatic datasets for our experiments. KEGG \citep{kanehisa2019toward, kanehisa2000kegg} is an enzymatic dataset containing compound and enzyme reaction data. BRENDA \citep{placzek2016brenda} is also an enzymatic dataset which contains human curated Enzyme Classification information in addition to inhibitor information. BindingDB \citep{gilson2016bindingdb} is a generic drug-target dataset. BindingDB comes in several flavors, we chose the BindingDB Purchasable dataset because it contains those compounds that have been experimentally demonstrated to be synthesizable for the listed reactions. We also establish a baseline using a model (GraphDTA) from \citep{nguyen2021graphdta} to measure performance against.

Methods:
%\begin{equation}
 %   \hat{y} = \sigma(MLP(z_{c1} \oplus z_{s2}) \oplus (z_{c2} \oplus z_{s1}))\label{eq17}
%\end{equation}
%where $\oplus$ is the concatenation operation. Both the compound based and the sequence based stratification can learn something unique from the data, therefore we used encoders trained from both stratification methods for final predictor training. 

%Assuming that $w_{neg}$ is the ratio of %negative-to-positive examples, where  $w_{neg} \geq 1$, %then the prediction loss, $l_n$, is defined as:
%\begin{equation}
%    l_n = -w_{neg} \times %log\frac{exp(\hat{y}_{n,y_n})}{exp(\hat{y}_{n,0}) + %exp(\hat{y}_{n,1})}\label{eq18}
%\end{equation}
%where $\hat{y}_{n,c}$ is the probability prediction for %$c^{th}$ class for $n^{th}$ example in the minibatch. The %final loss over the minibatch then is given by:
%\begin{equation}
%    L_{prediction} = %\Sigma^N_{n=1}\frac{1}{\Sigma^N_{n=1}w_{neg}}l_n\label{eq19}
%\end{equation}
%where N is the total number of examples in a minibatch.

%and K  s the number of known positive examples in a %minibatch.
%\begin{equation}
 %   N = K + w_{neg} * K\label{eq20}
%\end{equation}

%\subsection{CSI Model}\label{CSI_arch}
%The CSI model  for interaction prediction is trained in two phases (Figure \ref{fig:CSI_arch}).  
%In the first phase, encoders are trained on congruent views of the data, $V_C$ and $V_S$. The details of the molecule and sequence encoders are similar to the ones used in the baseline model from section \ref{baseline} to enable a reasonable comparison with the baseline. NN1 is the GCN based encoder for the compound. NN2 is a dual CNN based encoder for the pair of sequences. NN1 and NN2 are the encoders needed for equation \ref{eq1}. Similarly, NN3 is a dual GCN based encoder for the compounds and NN4 is the CNN based encoder for the sequence based on equation \ref{eq2}


%The CSI model explains the various encoders for different views of the data.
%For data stratified by compounds as explained in equation \ref{eq1}, NN1 is the encoder for the compound. NN2 contains two encoders for the sequences, followed by a concatenation layer. Similarly, for data stratified by sequence as described in equation \ref{eq2}, NN3 contains two encoders for the compounds, and NN4 is the encoder for the sequence. 
%In Phase 1 of the model, we use a contrastive loss to train the compound and protein embeddings.
%NN5 is an MLP layer using concatenated outputs from frozen NN1/NN2 and NN3/NN4.



%A molecule can be represented as a graph G with nodes $v \in V$ for the atoms, and edges $\{u,v\} \in E$ for the bonds. As in section \ref{baseline} We use a Graph Convolutional Network for learning the representation for the molecular graph. For a GCN, the message aggregation for the (i+1)th layer is given by \citep{kipf2016semi}
%\begin{equation}
 %   H^{(i+1)} = \sigma(\tilde{D}^{-\frac{1}{2}}\tilde{A}\tilde{D}^{-\frac{1}{2}}H^iW^i)\label{eq5}
%\end{equation}
%for $i = 1..K$ for a GCN with K layers. A is the Adjacency matrix of the graph, and $\tilde{A}$ is the Adjacency matrix with self loops. $\tilde{D}$ is the Diagonal matrix of $\tilde{A}$. $W^i$ are the weights for the i-th layer. In our case, we have a 3 layer GCN, so $K=3$. The final graph level embeddings are obtained by applying a MAXPOOL readout on the last layer of the GCN. For data stratified by compounds,
%\begin{equation}
 %   H_{compound} = MAXPOOL(H^K)\label{eq6}
%\end{equation}
%The final embeddings for the molecule are obtained by passing the above through %an MLP.
%\begin{equation}
%    h_{comp} = MLP(H_{compound})\label{eq7}
%\end{equation}
%\begin{equation}
%    z_{c1} = h_{comp}\label{eq8}
%\end{equation}

%For the protein sequence, we use a 1-dimensional CNN on the encoded FASTA sequence normalized to a fixed length (in our case, we used a length of 1000).
%\begin{equation}
%    H_{protein1} = CNN([MQT...PRS])\label{eq9}
%\end{equation}
%[MQT...PRS] is the protein FASTA sequence. The final embeddings for the sequence are obtained by passing the above through an MLP.
%\begin{equation}
 %   h_{protein1} = MLP(H_{protein1})\label{eq10}
%\end{equation}
%Similarly for protein 2,
%\begin{equation}
 %   H_{protein2} = CNN([MQT...PRS])\label{eq11}
%\end{equation}
%\begin{equation}
 %   h_{protein2} = MLP(H_{protein2})\label{eq12}
%\end{equation}
%\begin{equation}
%    z_{s2} = h_{protein1} \oplus h_{protein2}\label{eq13}
%\end{equation}



%The contrastive loss described below in equations \ref{eq14}, \ref{eq15} and \ref{eq16} is similar to the loss as described in \citep{tian2020contrastive} and over two views $V_1$ and $V_2$ is designed so as to move embeddings from congruent data closer in the latent space as explained in section \ref{intro}. We define a critic function $h_\theta$ is defined as the cosine similarity between the two encoders from equations \ref{eq8} and \ref{eq13} as:
%\begin{equation}
 %   h_\theta(v_i, v_j) = exp(\frac{z^i_{c1}.z^j_{s2}}{\|z^i_{c1}\|.\|z^j_{s2}\|}.\frac{1}{\tau})\label{eq14}
%\end{equation}
%$\tau$ is the temperature parameter which controls how aggressively we treat the non-congruent views.

%The contrastive loss over a minibatch is then given by
%\begin{equation}
 %   L^{V_1, V_2}_{contrastive} = -E[log\frac{h_\theta(z^1_{c1}, z^1_{s2})}{\Sigma^k_{j=2}h_\theta(z^1_{c1}, z^j_{s2})}]\label{eq15}
%\end{equation}
%k is the minibatch size. 

%Equation \ref{eq15} treats $V_1$ is the anchor view and iterates over $V_2$. Similarly we can anchor $V_2$ and iterate over $V_1$ to get $L^{V_2, V_1}_{contrastive}$. The total contrastive loss is then
%\begin{equation}
 %   L(V_1, V_2) = L^{V_1, V_2}_{contrastive} + L^{V_2, V_1}_{contrastive}\label{eq16}
%\end{equation}

%For sequence based stratification, similar embeddings $z_{c2}$ and $z_{s1}$ can be created by defining equations similar to equations \ref{eq6} - \ref{eq16}.

%


%\end{methods}

%\begin{methods}
%\section{Methods}

%\subsection{Contrastive Multiview Coding}\label{contrast}

%The mechanism to stratify and create multiple views of the same data, as explained in sections \ref{strat_inter} and \ref{strat_react} gives us the mechanism to apply CMC - as described in section \ref{intro}.  This can be visualized for both data schemes as shown in figure \ref{fig:contrast} below.
%The CSI (Contrastive Data Stratification for Interaction prediction) Model architecture pipeline is shown in Figure \ref{fig:CSI_arch}. 

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figs/contrast3.png}
    \caption{Contrastive Multiview Coding pushes embeddings for congruent data closer in a joint space. A) Interaction Data stratification followed by CMC B) Reaction data stratification followed by CMC}
    \label{fig:contrast}
\end{figure*}

Results:
%Looking at (Table \ref{tab:data_tab}) we can observe that a greater variance in compounds across data stratified by proteins in BindingDB ensures that the model sees a higher variety of compounds for BindingDB. The KEGG  dataset shows a higher variance in sequences.
